Follow the Curve: Robotic-Ultrasound Navigation with Learning Based Localization of Spinous Processes for Scoliosis Assessment

The scoliosis progression in adolescents requires close monitoring to timely take treatment measures. Ultrasound imaging is a radiation-free and low-cost alternative in scoliosis assessment to X-rays, which are typically used in clinical practice. However, ultrasound images are prone to speckle noises, making it challenging for sonographers to detect bony features and follow the spine's curvature. This paper introduces a robotic-ultrasound approach for spinal curvature tracking and automatic navigation. A fully connected network with deconvolutional heads is developed to locate the spinous process efficiently with real-time ultrasound images. We use this machine learning-based method to guide the motion of the robot-held ultrasound probe and follow the spinal curvature while capturing ultrasound images and correspondent position. We developed a new force-driven controller that automatically adjusts the probe's pose relative to the skin surface to ensure a good acoustic coupling between the probe and skin. After the scanning, the acquired data is used to reconstruct the coronal spinal image, where the deformity of the scoliosis spine can be assessed and measured. To evaluate the performance of our methodology, we conducted an experimental study with human subjects where the deviations from the image center during the robotized procedure are compared to that obtained from manual scanning. The angles of spinal deformity measured on spinal reconstruction images were similar for both methods, implying that they equally reflect human anatomy.

==> discussion.tex <==
\section{Discussion}
The spinous process localization algorithm yields excellent accuracy on the test dataset - 97.8\%. The method presents to be robust in defining the spinous process location with a mean distance error of 1.0mm. Spinous process continuous locations within Ultrasound scan of human back form a spinous process path, which can be used for the robotic navigation purpose. Kalman filter works well on filtering the outliers, wrongly detected as spinous process, and preventing the robot from sudden sideways movements. The filter also fills in the locations gaps where the predictions on intervertebral gaps give accuracy less than 0.5. 

The result of phantom scanning shows that the mean spinous process location among ultrasound frames was in $x_image = 322$ pixels, where the center of the ultrasound image is $x_image = 320$. Visually assessing the tracking results for phantom, in the Figure \ref{fig:tracking_results_phantom}, it is clear that the coronal image generated from the robotic scan has spine laying in the center of the field of view of the probe, the spinal features are more prominent, and the edges of the image are smoother. Since phantom is an idealistic case of the spine, and the network performance is pre-defined (since there is only one phantom in this study), it is necessary to run the test on a real human scenario. 

The human tracking results shows the mean of spinous process location is in $x_image = 328$ with $std=25$. It means that the method could maintain the spinous process in the middle of the ultrasound image during the entire scanning with an std of 25 pixels which corresponds to 3.1 mm. The coronal image of the robotic scan in Figure \ref{fig:tracking_results_human} illustrates that the spine is located in the center of the scan, and the image looks smooth. 

The region pitch rotation adjustment turned to be an essential improvement for the system. The higher rotations cannot be used if the subject has significant lordosis at the lumbar region due to the probe's shape. Then lower rotation gain should be used $r_x$. However, if the same subject has a highly curved upper back, the lower rotations will not be sufficient, and the probe will lose contact with the subject's back. Thus, region-specific pitch rotation can significantly improve the quality of resulted scanning images.

To investigate the performances of the spinal region's network, a model for 3 and 4 classes were used. However, both networks perform well according to accuracy; the network for 3 classes has an output more straightforward for the lumbar and thoracic region splitting. The robotic experiment with region-specific pitch rotation clearly shows the improvement in the resulted coronal image, Figure \ref{fig:region_spine_result_reconstruction_spine}. 

For the system validation and reliability assessment, the subject's trials will be conducted. It is also vital to determine user cases where robotic scanning is practical and the manual performs better, opening the path for future system improvements. 
